Problems with SZZ and Features: An empirical study of the state of practice of defect prediction data collection

Context: The SZZ algorithm is the de facto standard for labeling bug fixing commits and finding inducing changes for defect prediction data. Recent research uncovered potential problems in different parts of the SZZ algorithm. Most defect prediction data sets provide only static code metrics as features, while research indicates that other features are also important. Objective: We provide an empirical analysis of the defect labels created with the SZZ algorithm and the impact of commonly used features on results. Method: We used a combination of manual validation and adopted or improved heuristics for the collection of defect data. We conducted an empirical study on 398 releases of 38 Apache projects. Results: We found that only half of the bug fixing commits determined by SZZ are actually bug fixing. If a six-month time frame is used in combination with SZZ to determine which bugs affect a release, one file is incorrectly labeled as defective for every file that is correctly labeled as defective. In addition, two defective files are missed. We also explored the impact of the relatively small set of features that are available in most defect prediction data sets, as there are multiple publications that indicate that, e.g., churn related features are important for defect prediction. We found that the difference of using more features is not significant. Conclusion: Problems with inaccurate defect labels are a severe threat to the validity of the state of the art of defect prediction. Small feature sets seem to be a less severe threat.

==> noise.tex <==
\section{NOISE}

In comparison to prior work, we include changes from all development branches that are included in a release, i.e., not only changes on the main development branch, but also all changes on branches that were merged prior to the release. This follow the proposal by Kovalenko\etal~\cite{Kovalenko2018} to also include branch information in defect prediction data. 

The inclusion of branches in the change path is non-trivial, because we must keep track of the state of the code base in different branches. For example, the code base on a feature branch depends on the state of the code base when the branch was forked from the main development branch. We use a breadth first search to determine a consistent paths of commits that takes forks and merge commits into account. 


\subsection{Change Path Selection}
\label{sec:change_path_selection}
The selection of paths throughout the commit graph starts with selecting a slice of commits around the releases we are interested in. There are three ways for selecting these slices:

\begin{enumerate}
    \item Time, e.g., 6 months before and after the release.
    \item Number of commits, e.g., 250 commits before and after the release.
    \item Change size, e.g., all commits until 2500 lines changed before and after the release.
\end{enumerate}

We include all possible branches leading up to the release, i.e., all branches that are merged prior to the release. This gives us the most of the available data as mentioned by Kovalenko et al.~\cite{Kovalenko2018}.

To get every reachable commit from our target release we implemented standard breadth first search with two additions. 
The first one improves the algorithm by keeping track of branches so that we can follow complete paths of commits. This is important so that we do not jump between different states of the codebase, i.e., a commit on the master branch is followed by a commit on a feature branch where a lot of changes were already done. 
The second addition defines a break condition that terminates on commits younger that our target release commit date minus 6 months. This prevents us from traversing the complete graph back to the origin (or origins if multiple orphan commits exist).

\begin{figure}
    \begin{tikzpicture}[commit/.style={circle,draw,minimum width=0.5em, minimum height=0.5em, inner sep=1pt,-latex}]
        \node[commit] (release) {6};
        \node[commit, above left of = release] (c3) {3};
        \node[commit, left of = c3, dashed] (c2) {2};
        % \node[commit, left of = c2] (c1) {1};

        \node[commit, below left of = release] (l2) {5};
        \node[commit, left of = l2, dashed] (l1) {4};

        \node[commit, right of = release] (r1) {7};
        \node[commit, right of = r1, dashed] (r2) {8};


        % \draw[->] (c1) -- (c2) {};
        \draw[->,dashed] (c2) -- (c3) {};
        \draw[->] (c3) -- (release) {};

        \draw[->, dashed] (l1) -- (l2) {};
        \draw[->] (l2) -- (release) {};

        \draw[->] (release) -- (r1) {};
        \draw[->, dashed] (r1) -- (r2) {};

        % descriptions
        \node[below = 0cm of release] {1.0};

        % \node[above of = c1,align=left] {Bug A\\File 1};
        % \node[above of = c2,align=left] {Bug A\\File 2};
        \node[above = 0cm of c3,align=left] {\faBug};

        \node[below = 0cm of l2,align=left] {\faBug};
        % \node[below of = l2,align=left] {};

        \node[above = 0cm of r1,align=left] {\faBandAid};
        % \node[above of = r2,align=left] {Fix D};
    \end{tikzpicture}
    \caption{Defect labeling example}
    \label{fig:label}
\end{figure}

Figure~\ref{fig:label} shows an example of our approach. Given a target release, version 1.0 in the example, we add every bug-fixing commit that happened after the target release to a list of candidate bug-fixing commits.
From this list we examine each bug-fixing commit and its hunks, this gives us a list of files and the line numbers that changed in this commit, i.e. the lines for each file that fixed the bug.
For each file and each line we now use git blame functionality to find a list of candidates for commits that we label as bug-inducing.
From these candidates we now check if each of the commits has a path to our target release, commits 3 and 5 in Figure~\ref{fig:label} have a path to our release in commit 6.
If every bug-inducing commit happened before the target release and if each one has a path to the target release we count this as a bug-fix towards the file changed in commit 7.
